WassFFed: Wasserstein Fair Federated Learning

Federated Learning (FL) employs a training approach to address scenarios where users' data cannot be shared across clients. Achieving fairness in FL is imperative since training data in FL is inherently geographically distributed among diverse user groups. Existing research on fairness predominantly assumes access to the entire training data, making direct transfer to FL challenging. However, the limited existing research on fairness in FL does not effectively address two key challenges, i.e., (CH1) Current methods fail to deal with the inconsistency between fair optimization results obtained with surrogate functions and fair classification results. (CH2) Directly aggregating local fair models does not always yield a globally fair model due to non Identical and Independent data Distributions (non-IID) among clients. To address these challenges, we propose a Wasserstein Fair Federated Learning framework, namely WassFFed. To tackle CH1, we ensure that the outputs of local models, rather than the loss calculated with surrogate functions or classification results with a threshold, remain independent of various user groups. To resolve CH2, we employ a Wasserstein barycenter calculation of all local models' outputs for each user group, bringing local model outputs closer to the global output distribution to ensure consistency between the global model and local models. We conduct extensive experiments on three real-world datasets, demonstrating that WassFFed outperforms existing approaches in striking a balance between accuracy and fairness.

==> chapters/preliminary.tex <==
\section{Preliminary}
%
In this part, we first give the problem formulation.
%


==> tables/effect-of-clients.tex <==
\begin{table}\centering 
\renewcommand{\arraystretch}{1}
\caption{The effect of the number of clients}
\label{effect-of-client-table}
\begin{threeparttable}
\resizebox{\linewidth}{!}{
\begin{tabular}{rcccccc}
\hline
& \multicolumn{3}{c}{\M} & \multicolumn{3}{c}{FedAvg} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Clients & Acc ($\uparrow$) & $\mathcal{M}_{DP}$ ($\downarrow$) & $\mathcal{M}_{EOP}$ ($\downarrow$) & Acc ($\uparrow$) & $\mathcal{M}_{DP}$ ($\downarrow$) & $\mathcal{M}_{EOP}$ ($\downarrow$) \\ \hline  
2 & 0.6456 & 0.1949 &  0.1518 & 0.6622 & 0.3756 & 0.2411\\ 
4 & 0.6526 & 0.1697 & 0.1558 & 0.6646 & 0.3899 & 0.2363 \\
6 & 0.6503 & 0.1946 & 0.1654 & 0.6583 & 0.3897 & 0.2679 \\
8 & 0.6446 & 0.2001 & 0.1640 & 0.6503 & 0.3932 & 0.2756 \\
10 & 0.6433 & 0.2064 & 0.1732 & 0.6479 & 0.3979 & 0.2812 \\ 

\hline
\end{tabular}
}

    \end{threeparttable}
\end{table}


==> tables/experimental_results.tex <==
% \begin{table*}\centering 
% \renewcommand{\arraystretch}{1}
% \caption{Experimental result}
% \label{experiment-result-table}
% \begin{threeparttable}
% \begin{tabular}{clccccccccc}
% \hline
% \multicolumn{2}{c}{Dataset} & \multicolumn{3}{c}{Adult} & \multicolumn{3}{c}{Compas} & \multicolumn{3}{c}{Bank}  \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}

% $\alpha$ & \multicolumn{1}{c}{Method} & Acc ($\uparrow$) & SP ($\downarrow$) & EOP ($\downarrow$) & Acc ($\uparrow$) & SP ($\downarrow$) & EOP ($\downarrow$)  & Acc ($\uparrow$) & SP ($\downarrow$) & EOP ($\downarrow$) \\ \hline

% \multirow{5}{*}{0.5} & FedAvg & 81.92 & 12.31 & 23.42 & 68.22 & 33.88 & 36.94 & 88.15 & 2.51 & 0.91\\ 

% & AFL & 74.41 & 5.84 & 4.76 & 68.03 & 31.74 & 25.82 & 67.39 & 21.46 & 8.88\\

% & LocalFair & 77.23 & 3.30 & 1.09 & 67.84 & 32.20 & 34.27 & 88.27 & 0.00 & 0.00 \\

% & FedFB & 78.85 & 3.61 & 6.39 & 67.46 & 29.05 & 32.55 & 88.27 & 0.00 & 0.00 \\ 

% & WassFFed-local & 84.07 & 20.73 & 13.49 & 67.70 & 30.57 & 29.68 & 89.43 & 3.15 & 5.90 \\

% & \M & 78.09 & 3.13 & 7.03 & 64.93 & 19.81 & 21.31 & 88.27 & 0.00 & 0.00\\ \hline

% \multirow{5}{*}{5} & FedAvg & 84.47 & 22.59 & 21.52 & 68.51 & 32.98 & 36.60 & 89.10 & 8.36 & 2.24 \\

% & AFL & 75.92 & 3.62 & 1.98 & 66.93 & 33.42 & 25.69 & 88.90 & 0.31 & 1.94 \\

% & LocalFair & 82.23 & 16.98 & 37.12 & 68.34 & 32.26 & 34.24 & 88.27 & 0.00 & 0.00\\

% & FedFB & 84.07 & 20.73 & 13.49 & 68.37 & 29.29 & 25.24 & 89.43 & 3.15 & 5.90 \\

% & WassFFed-local & 84.07 & 20.73 & 13.49 & 68.17 & 30.41 & 25.32 & 89.43 & 3.15 & 5.90 \\

% & \M & 83.28 & 14.28 & 14.53 & 63.03 & 14.14 & 21.27 & 88.27 & 0.00 & 0.00 \\ \hline

% \multirow{5}{*}{100} & FedAvg & 84.72 & 21.40 & 22.16 & 68.65 & 32.59 & 36.65 & 89.30 & 7.55 & 2.48\\

% & AFL & 75.54 & 1.04 & 0.78 & 68.74 & 34.18 & 25.89 & 88.27 & 0.00 & 0.00 \\

% & LocalFair & 79.99 & 9.48 & 24.34 & 68.93 & 34.24 & 33.02 & 88.27 & 0.00 & 0.00 \\

% & FedFB & 84.03 & 21.60 & 15.04 &  67.74 & 31.43 & 27.68 & 88.27 & 0.00 & 0.00 \\

% & WassFFed-local & 84.07 & 20.73 & 13.49 & 68.08 & 31.90 & 36.74 & 89.43 & 3.15 & 5.90 \\
% & \M & 83.25 & 14.05 & 13.56 & 64.93 & 19.81 & 23.31 & 88.27 & 0.00 & 0.00 \\ \hline
% \end{tabular}

% \begin{tablenotes}
%         \footnotesize
%         \item[*] Note that the italic text indicates the result of UFR. The bold text indicates the result of our proposed \M~framework. The best results are marked with *.
%       \end{tablenotes}
%     \end{threeparttable}
% \end{table*}

\begin{table*}\centering 
\renewcommand{\arraystretch}{1}
\caption{Experimental result}
\vspace{-10pt}
\label{experiment-result-table}
\begin{threeparttable}
\begin{tabular}{clccccccccc}
\hline
& Dataset & \multicolumn{3}{c}{Adult} & \multicolumn{3}{c}{Compas} & \multicolumn{3}{c}{CelebA}  \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}

$\alpha$ & Method & Acc ($\uparrow$) & $\mathcal{M}_{DP}$ ($\downarrow$) & $\mathcal{M}_{EOP}$ ($\downarrow$) & Acc ($\uparrow$) & $\mathcal{M}_{DP}$ ($\downarrow$) & $\mathcal{M}_{EOP}$ ($\downarrow$)  & Acc ($\uparrow$) & $\mathcal{M}_{DP}$ ($\downarrow$) & $\mathcal{M}_{EOP}$ ($\downarrow$) \\ \hline

\multirow{5}{*}{0.5} & FedAvg & 0.8421* & 0.1534 & 0.1877 & 0.6646* & 0.3899 & 0.2363 & 0.8956* & 0.2819 & 0.1016 \\ 

& AFL & 0.7627 & \underline{0.0111} & \underline{0.0078} & 0.5944 & \underline{0.1907} & 0.1882 & 0.8247 & 0.2278  & \underline{0.0711} \\

& LocalFair & 0.7723 & 0.0330 & 0.0109 & 0.6019 & 0.2638 & \underline{0.1665} & 0.8752 & 0.2307 & 0.0999   \\

& FEDFB & 0.7567 & 0.0000* & 0.0000* & 0.6606 & 0.4092 & 0.2318 & \underline{0.8791} & 0.2390 & 0.0857  \\

& \MLocal & 0.8228 & 0.1336 & 0.2060 & \underline{0.6625} & 0.2171 & 0.3198 & 0.8867 & 0.1419* & 0.2480 \\ 

& \M & \textbf{\underline{0.8257}} & \textbf{0.1324} & \textbf{0.1136} & \textbf{0.6526} & \textbf{0.1697}* & \textbf{0.1558}* & \textbf{0.8715} & \textbf{\underline{0.1599}} & \textbf{0.0586}* \\ \hline

\multirow{5}{*}{5} & FedAvg & 0.8454* & 0.1690 & 0.2062 & \underline{0.6713} & 0.4364 & 0.2456 & \underline{0.9010} & 0.2961 & 0.1372  \\

& AFL & 0.7631 & 0.0000* & 0.0012* & 0.6152 & 0.2711 & 0.3040 & 0.8135 & 0.1662 & 0.0803   \\

& LocalFair & 0.8223 & 0.1698 & 0.3712 & 0.6019 & 0.2638 & \underline{0.1965} & 0.8913 & \underline{0.1432} & \underline{0.0734}  \\

& FEDFB & \underline{0.8407} & 0.1450 & 0.2000 & 0.6673 & 0.2735 & 0.2555 & 0.8887 & 0.1486 & 0.0805  \\

& \MLocal & 0.8273 & 0.1409 & 0.1525 & 0.6730* & \underline{0.2237} & 0.2957 & 0.8900 & 0.1694  & 0.0756 \\

& \M & \textbf{0.8393} & \textbf{\underline{0.1370}} & \textbf{\underline{0.1511}} & \textbf{0.6693} & \textbf{0.2210}* & \textbf{0.1906}* & \textbf{0.9035}* & \textbf{0.1319}* & \textbf{0.0675}* \\ \hline

\multirow{5}{*}{100} & FedAvg & 0.8455* & 0.1657 & 0.2078 & 0.6743* & 0.5291 & \underline{0.2433} & 0.9205* & 0.3314 & \underline{0.0743} \\

& AFL & 0.7633 & 0.0000* & 0.0031* & 0.6024 & 0.4527 & 0.3615 & 0.8647 & \underline{0.3008} & 0.0974  \\

& LocalFair & 0.7899 & \underline{0.0948} & 0.2434 & 0.6646 & 0.4765 & 0.3047 & 0.9025 & 0.3408 & 0.1455 \\

& FEDFB & \underline{0.8407} & 0.1472 & 0.1949 &  0.6730 & 0.5152 & 0.3544 & 0.9043 & 0.3372 & 0.0862  \\

& \MLocal & 0.8275 & 0.1404 & 0.1443 & \underline{0.6734} & \underline{0.2266} & 0.2985 & 0.8985 & 0.3208 & 0.0955 \\

& \M & \textbf{0.8396} & \textbf{0.1372} & \textbf{\underline{0.1379}} & \textbf{0.6706} & \textbf{0.2168}* & \textbf{0.1944}* & \textbf{\underline{0.9137}} & \textbf{0.2833}* & \textbf{0.0713}*   \\ \hline
\end{tabular}

\begin{tablenotes}
        \footnotesize
        \item[*] Note that the bold text indicates the result of our proposed \M~framework. The best results are marked with *. The second best results are underlined.
      \end{tablenotes}
    \end{threeparttable}
\end{table*}


% \begin{table*}\centering 
% \renewcommand{\arraystretch}{1}
% \caption{Experimental result}
% \label{ablation-table}
% \begin{threeparttable}
% \begin{tabular}{clccccccccc}
% \hline
% \multicolumn{2}{c}{} & \multicolumn{3}{c}{Adult clients=4} & \multicolumn{3}{c}{Compas clients=4} & \multicolumn{3}{c}{Celeba ResNet}  \\
% \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}

% {Method} & \multicolumn{1}{c}{$\alpha$} & Acc ($\uparrow$) & SP ($\downarrow$) & EOP ($\downarrow$) & Acc ($\uparrow$) & SP ($\downarrow$) & EOP ($\downarrow$)  & Acc ($\uparrow$) & SP ($\downarrow$) & EOP ($\downarrow$) \\ \hline

% \multirow{3}{*}{localWass} & 0.5 & 82.28 & 13.36 & 20.60 & 66.25 & 21.71 & 31.98 & 88.67 & 14.19 & 24.80 \\ 

% & 5 & 82.73 & 14.09 & 15.25 & 67.30 & 22.37 & 29.57 & 89.00 & 16.94  & 7.56 \\

% & 100 & 82.75 & 14.04 & 14.43 & 67.34 & 22.66 & 29.85 & 89.85 & 32.08 & 9.55   \\
% \hline

% \end{tabular}

% \begin{tablenotes}
%         \footnotesize
%         \item[*] Note that the italic text indicates the result of UFR. The bold text indicates the result of our proposed \M~framework. The best results are marked with *.
%       \end{tablenotes}
%     \end{threeparttable}
% \end{table*}
